MeshFlow: Mesh Generation with Equivariant Flow Matching

Meshes are among the most common 3D scene representations, but directly generating meshes is challenging because the representation contains important symmetries, including permutation invariance of faces and vertices. MeshFlow learns to generate triangle meshes directly as triangle soups, avoiding the need to serialize meshes into long autoregressive sequences. We adopt equivariant optimal-transport flow matching models that respect the key symmetries of triangle soups: arbitrary permutations of faces and permutations of the vertices within each face. Toward this goal, we propose a simple yet effective modification to the Diffusion Transformer architecture, resulting in a scalable network capable of modeling a velocity field while maintaining the desired equivariance. We further introduce an optimal-transport-based training objective that improves convergence by eliminating supervision signals that violate these symmetries. MeshFlow achieves mesh quality comparable to state-of-the-art autoregressive mesh generators while providing about an 18$\times$ speedup during inference. Project page is at https://qiisun.github.io/MeshFlow/.

==> figs/network.tex <==
\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{example-image-duck}
    \caption{Equivariant vertex network.}
    \label{fig:network}
\end{figure}

==> secs/7_figures.tex <==
\begin{figure*}[ht]
    \centering
\includegraphics[width=0.95\linewidth]{figs/comparison-sota.pdf}
    \caption{\textbf{Qualitative comparison with the-state-of-the-art methods.} }
    \label{fig:comparison-sota}
    \vspace{-1mm}
\end{figure*}


\begin{figure*}[ht]
    \centering
    \includegraphics[width=0.9\linewidth]{figs/ablation.pdf}
    \caption{\textbf{Analysis of Nested Optimal Transport.}
    Compared to independent coupling baseline, our nested OT achieves faster training convergence (a); better performance especially in   steps (b); and straighter intergral path (c).}
    \label{fig:ot-inf-vis}
\end{figure*}



\begin{figure}[ht]
    \centering
    \includegraphics[width=0.9\linewidth,]{figs/ablation-qualitive-2.pdf}
    \caption{\textbf{Qualitative results for ablative study.} Comparison between different data coupling (top row); comparison between different network architecture (bottom row).
    % \todo{Make it two rows}
    }
    \label{fig:nest-ot}
    % \vspace{-2mm}
\end{figure}


\begin{figure}[ht]
    \centering
    \includegraphics[width=0.9\linewidth]{figs/denoiser-1.pdf}
    \caption{\textbf{Impact of denoiser.} This learnable post-processing effectively removes the low-level noise in the raw model output.}
    \label{fig:denoiser}
    % \vspace{-1mm}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=0.9\linewidth]{figs/failure.pdf}
    \caption{\textbf{Failure cases.} }
    \label{fig:failure}
    % \vspace{-1mm}
\end{figure}


\begin{figure*}
    \centering
    \includegraphics[width=0.95\linewidth]{figs/gallery-final.pdf}
    \caption{\textbf{Gallery of our generated meshes.}}
    \label{fig:gallery}
\end{figure*}


==> tabs/ablation_eq.tex <==
\begin{table}[]
    \centering
        \caption{{Ablation study on equivariant network}.}
    \resizebox{0.85\linewidth}{!}{
    \begin{tabular}{lcccc}
    \toprule
       Method  &  MMD & COV & 1-NNA & JSD \\          \midrule
       % full equivariant network w/o mesh shuffle  & \\
       % full equivariant network variants & \\
       Face equivariant network & 18.2& 44.19& 72.42& 26.6\\
       Non-equivariant network & 20.8& 37.74& 83.87& 41.7
       \\
        Full equivariant network  & \textbf{17.1}& \textbf{49.0}& \textbf{55.97}& \textbf{11.5} \\
       \bottomrule
    \end{tabular}}
    \label{tab:ablation_network}
\end{table}

==> tabs/ablation_ot.tex <==
\begin{table}[]
    \centering
        \caption{Ablation study on data coupling methods.}
        \resizebox{0.8\linewidth}{!}{
    \begin{tabular}{lcccc}
    \toprule
         Method &  MMD  & COV & 1-NNA & JSD \\
         \midrule
    Independent coupling  & \textbf{16.9}& \textbf{54.52}& 57.42& 12.0\\
    Naive  coupling & 19.4 & 41.29&68.87 & 38.5\\
    Nested coupling  & 17.1& 49.0& \textbf{55.97}& \textbf{11.5}\\
       %  Independent coupling  &16.34 & 45.50  & 69.85 & 85.27\\
       % Naive  coupling & 13.20 & 59.50 &  67.57 & 58.42 \\
       % Nested coupling & \textbf{11.09} & \textbf{68.50} & \textbf{65.43} & \textbf{22.63} \\
       \bottomrule
    \end{tabular}}
    \label{tab:ablation_coupling}
    \vspace{-3mm}
\end{table}

==> tabs/ablation_time.tex <==
\begin{table}[]
    \centering
    \resizebox{0.5\textwidth}{!}{
    \begin{tabular}{lcccccc}
    \toprule
       Time scheduler  &  COV  & MMD & 1-NNA & JSD  & $R_f$ & $R_{if}$ \\     \midrule
       Uniform (0,1)  &  TT \\
       LN (0,1) & TT \\
       LN (0,1) + Shifted (8192) &  \\
       LN (0,1) + Shifted (64) & TE\\
       LN (0,1) + Shifted (32) & TE \\
       \bottomrule
    \end{tabular}
    }
    \caption{Effectiveness of face-dependent shifted temporal scheduler.}
    \label{tab:temporal-scheduler}
\end{table}
